Mass profiles and concentration-dark matter relation in X-ray luminous galaxy clusters

(Abriged) Assuming that the hydrostatic equilibrium holds between the intracluster medium and the gravitational potential, we constrain the NFW profiles in a sample of 44 X-ray luminous galaxy clusters observed with XMM-Newton in the redshift range 0.1-0.3. We evaluate several systematic uncertainties that affect our reconstruction of the X-ray masses. We measure the concentration c200, the dark mass M200 and the gas mass fraction within R500 in all the objects of our sample, providing the largest dataset of mass parameters for galaxy clusters in this redshift range. We confirm that a tight correlation between c200 and M200 is present and in good agreement with the predictions from numerical simulations and previous observations. When we consider a subsample of relaxed clusters that host a Low-Entropy-Core (LEC), we measure a flatter c-M relation with a total scatter that is lower by 40 per cent. From the distribution of the estimates of c200 and M200, with associated statistical (15-25%) and systematic (5-15%) errors, we use the predicted values from semi-analytic prescriptions calibrated through N-body numerical runs and measure sigma_8*Omega_m^(0.60+-0.03)= 0.45+-0.01 (at 2 sigma level, statistical only) for the subsample of the clusters where the mass reconstruction has been obtained more robustly, and sigma_8*Omega_m^(0.56+-0.04) = 0.39+-0.02 for the subsample of the 11 more relaxed LEC objects. With the further constraint from the fgas distribution in our sample, we break the degeneracy in the sigma_8-Omega_m plane and obtain the best-fit values sigma_8~1.0+-0.2 (0.75+-0.18 when the subsample of the more relaxed objects is considered) and Omega_m = 0.26+-0.01.

==> tab_cxo.tex <==
\begin{tabular}{l@{\hspace{.8em}} c@{\hspace{.7em}} c@{\hspace{.7em}} c@{\hspace{.7em}} c
 c@{\hspace{.7em}} c@{\hspace{.7em}} c@{\hspace{.7em}} c@{\hspace{.7em}} c@{\hspace{.7em}} c@{\hspace{.7em}} }
\hline \\
  & & & & & \multicolumn{6}{c}{{\it Method 1}} \\
 Cluster & z & ObsID & Instr & $t_{\rm exp}$ & $r_{\rm s}$ & $c_{200}$ & $M_{200}$ & $\chi_T^2$ (N) & $R_{500}$ & $f_{\rm gas}$ \\
         &   &       & & ksec & kpc & & $10^{14} M_{\odot}$ &  & kpc & $<R_{500}$  \\
\hline \\
Abell3827 & 0.098 & 7920 & ACIS-S & 45.3 & $558^{+134}_{-84}$ & $3.43^{+0.44}_{-0.50}$ & $5.85\pm0.51$ & $5.5 (9)$ & $921\pm28$ & $0.118\pm0.007$ \\
Abell2034 & 0.113 & 2204 & ACIS-I & 53.9 & $302^{+115}_{-67}$ & $5.65^{+1.32}_{-1.32}$ & $4.65\pm0.44$ & $8.7 (9)$ & $874\pm27$ & $0.123\pm0.009$ \\
Abell1068 & 0.138 & 1652 & ACIS-S & 26.8 & $314^{+30}_{-23}$ & $4.84^{+0.27}_{-0.30}$ & $3.29\pm0.18$ & $29.0 (9)$ & $760\pm16$ & $0.106\pm0.005$ \\
Abell1413 & 0.143 & 5003 & ACIS-I & 74.0 & $235^{+18}_{-26}$ & $6.75^{+0.69}_{-0.39}$ & $3.96\pm0.17$ & $10.1 (8)$ & $839\pm12$ & $0.151\pm0.006$ \\
RXCJ0547.6-3152 & 0.148 & 9419 & ACIS-I & 19.8 & $475^{+190}_{-72}$ & $3.77^{+0.53}_{-0.86}$ & $5.14\pm0.47$ & $0.7 (7)$ & $871\pm26$ & $0.113\pm0.008$ \\
Abell2204 & 0.152 & 499 & ACIS-S & 10.0 & $284^{+16}_{-22}$ & $6.32^{+0.36}_{-0.24}$ & $5.72\pm0.29$ & $13.8 (8)$ & $945\pm18$ & $0.155\pm0.006$ \\
Abell2218 & 0.176 & 1666 & ACIS-I & 41.2 & $245^{+103}_{-62}$ & $6.25^{+1.75}_{-1.59}$ & $3.63\pm0.36$ & $7.4 (7)$ & $803\pm25$ & $0.148\pm0.011$ \\
Abell1689 & 0.183 & 5004 & ACIS-I & 19.9 & $297^{+27}_{-21}$ & $6.58^{+0.39}_{-0.42}$ & $7.68\pm0.33$ & $15.4 (8)$ & $1021\pm16$ & $0.132\pm0.006$ \\
Abell383 & 0.187 & 524 & ACIS-I & 10.0 & $507^{+71}_{-23}$ & $3.69^{+0.13}_{-0.31}$ & $6.09\pm0.39$ & $8.1 (6)$ & $889\pm23$ & $0.077\pm0.005$ \\
Abell209 & 0.206 & 3579 & ACIS-I & 10.0 & $428^{+101}_{-101}$ & $3.81^{+0.99}_{-0.63}$ & $4.16\pm0.25$ & $11.5 (8)$ & $823\pm16$ & $0.169\pm0.008$ \\
Abell963 & 0.206 & 903 & ACIS-S & 36.3 & $407^{+144}_{-78}$ & $4.24^{+0.76}_{-0.86}$ & $5.03\pm0.57$ & $14.2 (7)$ & $857\pm34$ & $0.123\pm0.010$ \\
Abell773 & 0.217 & 5006 & ACIS-I & 19.6 & $514^{+228}_{-146}$ & $3.62^{+1.11}_{-0.91}$ & $6.17\pm0.69$ & $5.5 (7)$ & $912\pm33$ & $0.133\pm0.010$ \\
Abell1763 & 0.223 & 3591 & ACIS-I & 19.6 & $116^{+38}_{-16}$ & $11.66^{+1.47}_{-2.57}$ & $2.85\pm0.19$ & $2.5 (8)$ & $758\pm16$ & $0.191\pm0.011$ \\
Abell2390 & 0.228 & 4193 & ACIS-S & 91.2 & $1261^{+0}_{-209}$ & $2.06^{+0.27}_{-0.04}$ & $14.68\pm0.92$ & $8.0 (8)$ & $1159\pm32$ & $0.124\pm0.006$ \\
RXCJ2129.6+0005 & 0.235 & 552 & ACIS-I & 10.0 & $328^{+24}_{-22}$ & $4.65^{+0.26}_{-0.25}$ & $3.64\pm0.14$ & $2.7 (6)$ & $782\pm11$ & $0.161\pm0.006$ \\
Abell1835 & 0.253 & 495 & ACIS-S & 19.5 & $469^{+49}_{-31}$ & $4.24^{+0.20}_{-0.28}$ & $8.13\pm0.44$ & $10.5 (7)$ & $1004\pm20$ & $0.149\pm0.007$ \\
RXCJ0307.0-2840 & 0.253 & 9414 & ACIS-I & 18.9 & $331^{+98}_{-68}$ & $5.11^{+1.02}_{-0.94}$ & $5.17\pm0.57$ & $5.1 (7)$ & $861\pm33$ & $0.129\pm0.011$ \\
Abell68 & 0.255 & 3250 & ACIS-I & 10.0 & $511^{+155}_{-89}$ & $3.80^{+0.65}_{-0.75}$ & $7.40\pm0.50$ & $11.9 (6)$ & $948\pm22$ & $0.115\pm0.006$ \\
E1455+2232 & 0.258 & 4192 & ACIS-I & 91.1 & $180^{+16}_{-11}$ & $7.18^{+0.34}_{-0.42}$ & $2.44\pm0.12$ & $3.8 (6)$ & $693\pm12$ & $0.167\pm0.008$ \\
RXCJ0232.2-4420 & 0.284 & 4993 & ACIS-I & 22.6 & $610^{+376}_{-190}$ & $2.88^{+0.97}_{-0.88}$ & $5.30\pm0.84$ & $18.6 (7)$ & $855\pm45$ & $0.173\pm0.017$ \\
ZW3146 & 0.291 & 909 & ACIS-I & 46.0 & $442^{+27}_{-26}$ & $3.97^{+0.18}_{-0.16}$ & $5.72\pm0.22$ & $8.5 (6)$ & $880\pm12$ & $0.152\pm0.006$ \\
RXCJ0043.4-2037 & 0.292 & 9409 & ACIS-I & 19.9 & $273^{+167}_{-138}$ & $5.68^{+4.76}_{-1.88}$ & $4.22\pm0.64$ & $10.3 (6)$ & $811\pm37$ & $0.159\pm0.016$ \\
\hline \\
\end{tabular}


==> tab_m1m2_m200.tex <==
\begin{tabular}{l@{\hspace{.8em}} c@{\hspace{.7em}} c@{\hspace{.8em}} 
 c@{\hspace{.8em}} c@{\hspace{.7em}} c@{\hspace{.7em}} c@{\hspace{.8em}}
 c@{\hspace{.8em}} c@{\hspace{.7em}} c@{\hspace{.7em}} c@{\hspace{.8em}} }
\hline \\
 Cluster & z & Instr & $M_{200}$ & $c_{200}$ & $f_{\rm gas, 200}$ & $\chi_T^2$ (N) & 
    $\hat{M}_{200}$ & $\hat{c}_{200}$ & $\hat{f}_{\rm gas, 200}$ & $\chi_T^2$ (N) \\ 
    &  &  &  $10^{14} M_{\odot}$ &  & & & $10^{14} M_{\odot}$ &   \\
\hline \\
RXCJ0003.8+0203 & 0.092 & M1 & $5.49\pm1.08$ & $3.54\pm0.74$ & $0.086\pm0.017$ & $1.8 (7)$ & $1.52\pm0.51$ & $9.25\pm3.73$ & $0.169\pm0.057$ & $3.3 (7)$ \\
Abell3911 & 0.097 & M2 & $8.06\pm1.70$ & $2.65\pm0.89$ & $0.121\pm0.026$ & $13.1 (9)$ & $6.38\pm2.15$ & $3.78\pm1.78$ & $0.141\pm0.048$ & $17.2 (9)$ \\
Abell3827 & 0.098 & M1 & $17.10\pm2.43$ & $2.74\pm0.42$ & $0.089\pm0.013$ & $1.8 (9)$ & $9.06\pm2.27$ & $3.63\pm1.01$ & $0.150\pm0.038$ & $5.0 (9)$ \\
RXCJ0049.4-2931 & 0.108 & M2 & $1.27\pm0.69$ & $7.33\pm4.52$ & $0.162\pm0.087$ & $3.1 (6)$ & $0.47\pm0.14$ & $19.42\pm5.00$ & $0.278\pm0.081$ & $14.8 (6)$ \\
Abell2034 & 0.113 & M2 & $17.30\pm2.55$ & $2.42\pm0.41$ & $0.074\pm0.011$ & $3.3 (9)$ & $12.50\pm5.43$ & $4.35\pm2.38$ & $0.106\pm0.046$ & $3.3 (9)$ \\
RXCJ1516.5-0056 & 0.115 & M2 & $5.16\pm0.99$ & $2.83\pm0.57$ & $0.110\pm0.021$ & $3.8 (7)$ & $6.77\pm1.30$ & $3.13\pm0.65$ & $0.104\pm0.020$ & $9.5 (7)$ \\
RXCJ1516.3+0005 & 0.118 & M1 & $2.84\pm1.14$ & $6.57\pm3.10$ & $0.166\pm0.067$ & $3.1 (7)$ & $8.50\pm1.67$ & $3.26\pm0.77$ & $0.075\pm0.015$ & $3.3 (7)$ \\
RXCJ2149.1-3041 & 0.118 & M2 & $5.39\pm0.85$ & $2.83\pm0.42$ & $0.086\pm0.014$ & $5.6 (7)$ & $4.63\pm1.01$ & $3.14\pm0.61$ & $0.088\pm0.019$ & $6.0 (7)$ \\
RXCJ1141.4-1216 & 0.119 & M1 & $5.95\pm0.73$ & $2.93\pm0.31$ & $0.083\pm0.010$ & $4.2 (7)$ & $6.01\pm0.29$ & $2.88\pm0.08$ & $0.088\pm0.004$ & $9.0 (7)$ \\
RXCJ1044.5-0704 & 0.132 & M1 & $7.11\pm0.91$ & $2.88\pm0.33$ & $0.081\pm0.010$ & $5.6 (7)$ & $6.46\pm0.30$ & $2.69\pm0.09$ & $0.100\pm0.005$ & $22.7 (7)$ \\
Abell1068 & 0.138 & M2 & $8.51\pm1.31$ & $2.55\pm0.32$ & $0.075\pm0.012$ & $9.7 (9)$ & $5.51\pm1.58$ & $3.19\pm0.68$ & $0.104\pm0.030$ & $7.3 (8)$ \\
RXCJ2218.6-3853 & 0.138 & M2 & $10.40\pm1.07$ & $3.04\pm0.26$ & $0.101\pm0.010$ & $5.7 (7)$ & $8.81\pm3.14$ & $3.59\pm1.71$ & $0.090\pm0.032$ & $5.9 (7)$ \\
RXCJ0605.8-3518 & 0.141 & M2 & $8.94\pm0.66$ & $2.83\pm0.15$ & $0.060\pm0.004$ & $4.4 (7)$ & $9.28\pm0.75$ & $2.88\pm0.18$ & $0.094\pm0.008$ & $17.6 (7)$ \\
RXCJ0020.7-2542 & 0.142 & M2 & $16.20\pm3.70$ & $3.49\pm1.05$ & $0.031\pm0.007$ & $0.7 (7)$ & $15.80\pm2.75$ & $3.39\pm0.58$ & $0.049\pm0.009$ & $6.6 (7)$ \\
Abell1413 & 0.143 & M2 & $13.30\pm2.94$ & $3.24\pm0.68$ & $0.101\pm0.022$ & $4.9 (8)$ & $23.60\pm2.26$ & $2.93\pm0.25$ & $0.064\pm0.006$ & $12.6 (8)$ \\
RXCJ2048.1-1750 & 0.147 & M2 & $6.58\pm1.28$ & $2.46\pm0.56$ & $0.136\pm0.026$ & $10.2 (7)$ & $6.58\pm1.28$ & $2.46\pm0.61$ & $0.134\pm0.026$ & $12.1 (7)$ \\
RXCJ0547.6-3152 & 0.148 & M1 & $13.20\pm2.01$ & $3.09\pm0.48$ & $0.082\pm0.012$ & $2.1 (7)$ & $10.90\pm1.92$ & $2.93\pm0.61$ & $0.108\pm0.019$ & $5.6 (7)$ \\
Abell2204 & 0.152 & M1 & $20.90\pm0.74$ & $2.64\pm0.05$ & $0.097\pm0.003$ & $24.3 (8)$ & $19.80\pm0.79$ & $2.59\pm0.07$ & $0.100\pm0.004$ & $27.0 (8)$ \\
RXCJ2234.5-3744 & 0.153 & M2 & $18.60\pm5.36$ & $3.47\pm1.51$ & $0.059\pm0.017$ & $0.9 (7)$ & $9.14\pm5.03$ & $4.65\pm3.67$ & $0.108\pm0.060$ & $8.3 (7)$ \\
RXCJ0958.3-1103 & 0.153 & M2 & $9.48\pm1.81$ & $2.69\pm0.50$ & $0.093\pm0.018$ & $3.1 (7)$ & $9.35\pm0.96$ & $2.68\pm0.18$ & $0.102\pm0.010$ & $14.6 (7)$ \\
RXCJ2014.8-2430 & 0.161 & M1 & $17.60\pm2.62$ & $2.55\pm0.32$ & $0.096\pm0.014$ & $4.7 (8)$ & $13.40\pm0.62$ & $2.88\pm0.08$ & $0.111\pm0.005$ & $5.5 (7)$ \\
RXCJ0645.4-5413 & 0.167 & M1 & $21.00\pm6.73$ & $2.43\pm1.12$ & $0.097\pm0.031$ & $1.1 (8)$ & $6.19\pm2.95$ & $4.26\pm2.55$ & $0.229\pm0.109$ & $4.0 (8)$ \\
Abell2218 & 0.176 & M2 & $4.92\pm2.92$ & $5.61\pm3.97$ & $0.189\pm0.112$ & $0.7 (7)$ & $13.60\pm3.11$ & $2.71\pm0.87$ & $0.097\pm0.022$ & $6.0 (7)$ \\
Abell1689 & 0.183 & M2 & $19.20\pm3.66$ & $3.63\pm0.60$ & $0.100\pm0.019$ & $2.0 (8)$ & $32.50\pm2.95$ & $3.52\pm0.24$ & $0.063\pm0.006$ & $15.9 (7)$ \\
Abell383 & 0.187 & M2 & $7.67\pm0.93$ & $2.74\pm0.31$ & $0.087\pm0.011$ & $3.5 (6)$ & $7.59\pm0.38$ & $2.69\pm0.08$ & $0.070\pm0.004$ & $22.3 (6)$ \\
Abell209 & 0.206 & M1 & $18.90\pm2.84$ & $1.98\pm0.37$ & $0.109\pm0.016$ & $5.2 (8)$ & $18.30\pm1.51$ & $1.94\pm0.12$ & $0.124\pm0.010$ & $19.4 (8)$ \\
Abell963 & 0.206 & M2 & $12.50\pm2.66$ & $2.42\pm0.66$ & $0.092\pm0.020$ & $1.4 (7)$ & $9.02\pm3.01$ & $3.64\pm1.28$ & $0.118\pm0.040$ & $3.3 (7)$ \\
Abell773 & 0.217 & M2 & $18.60\pm3.06$ & $2.51\pm0.44$ & $0.086\pm0.014$ & $5.4 (7)$ & $15.90\pm6.45$ & $2.68\pm2.33$ & $0.111\pm0.045$ & $6.8 (7)$ \\
Abell1763 & 0.223 & M2 & $12.80\pm4.17$ & $2.37\pm1.28$ & $0.161\pm0.052$ & $2.3 (8)$ & $3.41\pm1.49$ & $12.13\pm7.45$ & $0.368\pm0.161$ & $6.8 (8)$ \\
Abell2390 & 0.228 & M1 & $25.20\pm4.16$ & $1.98\pm0.25$ & $0.122\pm0.020$ & $14.5 (8)$ & $19.40\pm2.35$ & $2.42\pm0.22$ & $0.137\pm0.016$ & $12.0 (7)$ \\
Abell2667 & 0.230 & M2 & $16.70\pm1.02$ & $2.29\pm0.10$ & $0.101\pm0.006$ & $12.8 (7)$ & $15.10\pm0.83$ & $2.21\pm0.08$ & $0.106\pm0.006$ & $19.4 (7)$ \\
RXJ2129.6+0005 & 0.235 & M1 & $10.30\pm0.51$ & $2.46\pm0.11$ & $0.130\pm0.006$ & $3.1 (6)$ & $9.67\pm0.36$ & $2.42\pm0.06$ & $0.132\pm0.005$ & $15.9 (6)$ \\
RXCJ0307.0-2840 & 0.253 & M1 & $17.80\pm3.86$ & $2.18\pm0.51$ & $0.090\pm0.020$ & $2.6 (7)$ & $6.85\pm2.88$ & $4.13\pm1.97$ & $0.175\pm0.074$ & $9.5 (7)$ \\
Abell1835 & 0.253 & M1 & $23.90\pm0.87$ & $2.38\pm0.05$ & $0.094\pm0.003$ & $17.9 (7)$ & $20.20\pm0.85$ & $2.29\pm0.06$ & $0.098\pm0.004$ & $24.6 (7)$ \\
Abell68 & 0.255 & M2 & $9.79\pm3.57$ & $3.69\pm1.95$ & $0.122\pm0.044$ & $6.9 (6)$ & $18.40\pm2.00$ & $2.79\pm0.23$ & $0.065\pm0.007$ & $9.2 (6)$ \\
E1455+2232 & 0.258 & M2 & $9.80\pm1.65$ & $2.59\pm0.42$ & $0.106\pm0.018$ & $0.6 (6)$ & $7.40\pm2.05$ & $3.39\pm0.83$ & $0.118\pm0.033$ & $1.4 (6)$ \\
RXCJ2337.6+0016 & 0.273 & M2 & $13.00\pm5.77$ & $2.54\pm3.10$ & $0.112\pm0.050$ & $3.1 (7)$ & $8.90\pm4.05$ & $3.04\pm2.36$ & $0.161\pm0.073$ & $7.1 (7)$ \\
RXCJ0303.8-7752 & 0.274 & M1 & $15.90\pm4.80$ & $1.96\pm0.90$ & $0.111\pm0.033$ & $3.1 (7)$ & $1.95\pm0.61$ & $19.62\pm5.41$ & $0.400\pm0.124$ & $14.0 (6)$ \\
RXCJ0532.9-3701 & 0.275 & M2 & $10.40\pm5.42$ & $3.49\pm2.94$ & $0.134\pm0.070$ & $2.8 (6)$ & $11.70\pm5.66$ & $3.69\pm2.49$ & $0.106\pm0.051$ & $10.7 (6)$ \\
RXCJ0232.4-4420 & 0.284 & M2 & $15.20\pm3.91$ & $1.90\pm0.71$ & $0.117\pm0.030$ & $8.7 (7)$ & $13.30\pm2.34$ & $2.29\pm0.39$ & $0.107\pm0.019$ & $4.4 (6)$ \\
ZW3146 & 0.291 & M2 & $12.50\pm0.57$ & $2.29\pm0.07$ & $0.115\pm0.005$ & $9.9 (6)$ & $15.00\pm0.29$ & $2.34\pm0.03$ & $0.099\pm0.002$ & $30.2 (6)$ \\
RXCJ0043.4-2037 & 0.292 & M1 & $11.30\pm5.78$ & $3.11\pm3.24$ & $0.145\pm0.074$ & $3.9 (6)$ & $15.70\pm3.63$ & $2.36\pm0.80$ & $0.099\pm0.023$ & $8.5 (6)$ \\
RXCJ0516.7-5430 & 0.295 & M2 & $11.00\pm3.28$ & $1.71\pm1.80$ & $0.210\pm0.063$ & $3.5 (7)$ & $0.70\pm0.40$ & $19.42\pm8.54$ & $0.764\pm0.435$ & $13.5 (7)$ \\
RXCJ1131.9-1955 & 0.307 & M1 & $24.80\pm4.06$ & $2.06\pm0.35$ & $0.120\pm0.020$ & $3.5 (7)$ & $12.90\pm2.62$ & $1.67\pm0.47$ & $0.174\pm0.036$ & $6.0 (7)$ \\
\end{tabular}


==> tab_m200.tex <==
\begin{tabular}{l@{\hspace{.8em}} c@{\hspace{.7em}} c@{\hspace{.8em}} c@{\hspace{.7em}}
 c@{\hspace{.8em}} c@{\hspace{.7em}} c@{\hspace{.7em}} c@{\hspace{.8em}} }
\hline \\
 Cluster & z & $R_{\rm xsp}$ & $r_{\rm s}$ & $c_{200}$ & $M_{200}$ & $f_{\rm gas, 200}$ & $\chi_T^2$ (N) \\
    &  & kpc & kpc &  & $10^{14} M_{\odot}$ &   \\
\hline \\
RXCJ0003.8+0203 & 0.092 & $414$ & $143^{+36}_{-28}$ & $8.06^{+1.52}_{-1.30}$ & $1.90\pm0.23$ & $0.147\pm0.063$ & $2.3 (7)$ \\
Abell3911 & 0.097 & $754$ & $261^{+108}_{-59}$ & $5.59^{+1.33}_{-1.39}$ & $3.88\pm0.50$ & $0.178\pm0.059$ & $10.2 (9)$ \\
Abell3827 & 0.098 & $767$ & $390^{+89}_{-64}$ & $4.47^{+0.67}_{-0.64}$ & $6.61\pm0.73$ & $0.171\pm0.017$ & $3.4 (9)$ \\
RXCJ0049.4-2931 & 0.108 & $371$ & $71^{+30}_{-19}$ & $12.77^{+3.80}_{-3.18}$ & $0.94\pm0.16$ & $0.176\pm0.027$ & $5.7 (6)$ \\
Abell2034 & 0.113 & $866$ & $979^{+7}_{-317}$ & $2.46^{+0.81}_{-0.06}$ & $17.64\pm2.17$ & $0.070\pm0.009$ & $7.7 (9)$ \\
RXCJ1516.5-0056 & 0.115 & $502$ & $563^{+0}_{-114}$ & $2.75^{+0.49}_{-0.06}$ & $4.73\pm0.42$ & $0.143\pm0.014$ & $8.1 (7)$ \\
RXCJ2149.1-3041 & 0.118 & $513$ & $251^{+41}_{-28}$ & $4.79^{+0.43}_{-0.49}$ & $2.21\pm0.21$ & $0.161\pm0.034$ & $24.6 (7)$ \\
RXCJ1516.3+0005 & 0.118 & $514$ & $185^{+67}_{-42}$ & $7.06^{+1.64}_{-1.54}$ & $2.84\pm0.41$ & $0.176\pm0.092$ & $2.8 (7)$ \\
RXCJ1141.4-1216 & 0.119 & $519$ & $496^{+60}_{-36}$ & $3.15^{+0.19}_{-0.24}$ & $4.88\pm0.37$ & $0.091\pm0.013$ & $13.0 (7)$ \\
RXCJ1044.5-0704 & 0.132 & $566$ & $286^{+23}_{-27}$ & $4.56^{+0.34}_{-0.25}$ & $2.86\pm0.18$ & $0.148\pm0.019$ & $13.3 (7)$ \\
Abell1068 & 0.138 & $1026$ & $564^{+66}_{-49}$ & $3.02^{+0.20}_{-0.22}$ & $6.40\pm0.48$ & $0.083\pm0.007$ & $8.0 (9)$ \\
RXCJ2218.6-3853 & 0.138 & $587$ & $597^{+184}_{-166}$ & $3.16^{+0.85}_{-0.55}$ & $8.76\pm1.62$ & $0.107\pm0.022$ & $9.9 (7)$ \\
RXCJ0605.8-3518 & 0.141 & $598$ & $369^{+47}_{-39}$ & $4.10^{+0.34}_{-0.34}$ & $4.51\pm0.36$ & $0.134\pm0.057$ & $17.8 (7)$ \\
RXCJ0020.7-2542 & 0.142 & $603$ & $473^{+245}_{-154}$ & $4.17^{+1.41}_{-1.07}$ & $10.03\pm2.67$ & $0.055\pm0.017$ & $17.7 (7)$ \\
Abell1413 & 0.143 & $793$ & $287^{+23}_{-32}$ & $5.83^{+0.57}_{-0.35}$ & $6.12\pm0.32$ & $0.196\pm0.061$ & $6.3 (8)$ \\
RXCJ2048.1-1750 & 0.147 & $619$ & $742^{+80}_{-370}$ & $2.23^{+1.63}_{-0.21}$ & $5.96\pm1.12$ & $0.147\pm0.052$ & $2.7 (7)$ \\
RXCJ0547.6-3152 & 0.148 & $624$ & $443^{+253}_{-71}$ & $4.10^{+0.59}_{-1.17}$ & $7.89\pm1.51$ & $0.117\pm0.065$ & $4.7 (7)$ \\
Abell2204 & 0.152 & $837$ & $816^{+137}_{-0}$ & $2.81^{+0.02}_{-0.28}$ & $15.93\pm1.19$ & $0.129\pm0.010$ & $58.3 (8)$ \\
RXCJ0958.3-1103 & 0.153 & $639$ & $872^{+260}_{-183}$ & $2.39^{+0.42}_{-0.39}$ & $11.94\pm2.02$ & $0.091\pm0.042$ & $3.8 (7)$ \\
RXCJ2234.5-3744 & 0.153 & $640$ & $506^{+261}_{-220}$ & $4.28^{+2.31}_{-1.16}$ & $13.42\pm4.15$ & $0.070\pm0.060$ & $1.4 (7)$ \\
RXCJ2014.8-2430 & 0.161 & $878$ & $462^{+59}_{-25}$ & $3.86^{+0.15}_{-0.30}$ & $7.56\pm0.53$ & $0.165\pm0.018$ & $28.6 (8)$ \\
RXCJ0645.4-5413 & 0.167 & $904$ & $380^{+135}_{-89}$ & $4.58^{+1.06}_{-0.96}$ & $7.08\pm1.12$ & $0.197\pm0.082$ & $7.7 (8)$ \\
Abell2218 & 0.176 & $716$ & $243^{+95}_{-79}$ & $6.26^{+2.46}_{-1.48}$ & $4.76\pm0.74$ & $0.199\pm0.099$ & $11.3 (7)$ \\
Abell1689 & 0.183 & $974$ & $211^{+22}_{-19}$ & $8.31^{+0.64}_{-0.63}$ & $7.36\pm0.44$ & $0.168\pm0.009$ & $16.3 (8)$ \\
Abell383 & 0.187 & $589$ & $435^{+95}_{-0}$ & $3.40^{+0.03}_{-0.42}$ & $4.43\pm0.37$ & $0.130\pm0.078$ & $27.0 (6)$ \\
Abell209 & 0.206 & $1069$ & $604^{+272}_{-133}$ & $3.03^{+0.67}_{-0.77}$ & $8.60\pm1.23$ & $0.175\pm0.034$ & $8.8 (8)$ \\
Abell963 & 0.206 & $813$ & $377^{+107}_{-83}$ & $4.35^{+0.94}_{-0.76}$ & $6.17\pm0.83$ & $0.134\pm0.034$ & $5.7 (7)$ \\
Abell773 & 0.217 & $846$ & $605^{+408}_{-233}$ & $3.27^{+1.49}_{-1.05}$ & $10.94\pm3.12$ & $0.122\pm0.064$ & $6.6 (7)$ \\
Abell1763 & 0.223 & $1136$ & $192^{+194}_{-49}$ & $7.50^{+2.30}_{-3.41}$ & $4.25\pm0.74$ & $0.272\pm0.042$ & $8.1 (8)$ \\
Abell2390 & 0.228 & $1156$ & $1258^{+0}_{-95}$ & $2.06^{+0.12}_{-0.04}$ & $24.71\pm1.16$ & $0.106\pm0.020$ & $11.6 (8)$ \\
Abell2667 & 0.230 & $885$ & $993^{+0}_{-48}$ & $2.24^{+0.08}_{-0.02}$ & $15.88\pm0.45$ & $0.119\pm0.019$ & $4.8 (7)$ \\
RXCJ2129.6+0005 & 0.235 & $702$ & $418^{+68}_{-37}$ & $3.71^{+0.27}_{-0.38}$ & $5.40\pm0.44$ & $0.192\pm0.033$ & $3.4 (6)$ \\
Abell1835 & 0.253 & $950$ & $866^{+46}_{-143}$ & $2.64^{+0.34}_{-0.09}$ & $17.53\pm1.41$ & $0.123\pm0.015$ & $10.9 (7)$ \\
RXCJ0307.0-2840 & 0.253 & $951$ & $611^{+297}_{-175}$ & $3.15^{+0.88}_{-0.78}$ & $10.44\pm2.39$ & $0.110\pm0.023$ & $5.0 (7)$ \\
Abell68 & 0.255 & $746$ & $834^{+0}_{-257}$ & $2.65^{+0.82}_{-0.06}$ & $15.96\pm1.97$ & $0.071\pm0.009$ & $4.4 (6)$ \\
E1455+2232 & 0.258 & $752$ & $214^{+26}_{-22}$ & $6.32^{+0.53}_{-0.51}$ & $3.66\pm0.29$ & $0.195\pm0.025$ & $2.7 (6)$ \\
RXCJ2337.6+0016 & 0.273 & $1004$ & $332^{+342}_{-154}$ & $4.99^{+3.52}_{-2.18}$ & $6.81\pm1.91$ & $0.152\pm0.039$ & $1.1 (7)$ \\
RXCJ0303.8-7752 & 0.274 & $1007$ & $1115^{+14}_{-497}$ & $1.85^{+1.04}_{-0.09}$ & $13.21\pm2.33$ & $0.112\pm0.019$ & $5.7 (7)$ \\
RXCJ0532.9-3701 & 0.275 & $787$ & $278^{+170}_{-98}$ & $5.97^{+2.43}_{-1.82}$ & $6.88\pm1.83$ & $0.155\pm0.037$ & $3.3 (6)$ \\
RXCJ0232.2-4420 & 0.284 & $1032$ & $1172^{+0}_{-409}$ & $1.80^{+0.66}_{-0.04}$ & $14.28\pm1.90$ & $0.102\pm0.036$ & $12.4 (7)$ \\
ZW3146 & 0.291 & $820$ & $510^{+61}_{-31}$ & $3.37^{+0.15}_{-0.26}$ & $7.79\pm0.49$ & $0.171\pm0.020$ & $27.5 (6)$ \\
RXCJ0043.4-2037 & 0.292 & $823$ & $186^{+196}_{-81}$ & $7.80^{+5.05}_{-3.51}$ & $4.70\pm1.24$ & $0.213\pm0.063$ & $10.7 (6)$ \\
RXCJ0516.7-5430 & 0.295 & $1061$ & $785^{+405}_{-472}$ & $2.41^{+2.82}_{-0.75}$ & $10.44\pm2.88$ & $0.133\pm0.034$ & $1.8 (7)$ \\
RXCJ1131.9-1955 & 0.307 & $1091$ & $797^{+494}_{-309}$ & $2.43^{+1.16}_{-0.76}$ & $11.31\pm2.50$ & $0.172\pm0.040$ & $6.9 (7)$ \\
\hline \\
\end{tabular}

